Run Like a Girl! Sports-Related Gender Bias in Language and Vision

Gender bias in Language and Vision datasets and models has the potential to perpetuate harmful stereotypes and discrimination. We analyze gender bias in two Language and Vision datasets. Consistent with prior work, we find that both datasets underrepresent women, which promotes their invisibilization. Moreover, we hypothesize and find that a bias affects human naming choices for people playing sports: speakers produce names indicating the sport (e.g. 'tennis player' or 'surfer') more often when it is a man or a boy participating in the sport than when it is a woman or a girl, with an average of 46% vs. 35% of sports-related names for each gender. A computational model trained on these naming data reproduces the bias. We argue that both the data and the model result in representational harm against women.

==> discussion-legacy.tex <==


%\EG{Overall conclusion: we stress that it is important to have balanced datasets to avoid biased models. We report the finding of this - previously unnoticed - bias in human naming annotations: this must be taken into account when training models to output labels for objects. Something brief about the fact that we cannot get unbiased annotations until we remove bias from society.}%


%Humans are flawed creatures. We each possess our own biases and the insidious nature of implicit bias is why we can be so unaware of its very existence in our lives \cite{Haselton2015}.
%Sports are historically and culturally segregated \cite{Dennis2015} in addition to being one of the most observable manifestations of gender bias and discrimination. %While in other fields, bias is visible in socioeconomic indicators such as salary and position, in sports the bias is at the bodily level \cite{Young1980}, \cite{Straus1952}, \cite{Bourdieu2000}. By using the sports discrepancies within the gender we are able to see the discrimination at the least abstract level. In Straus' \cite{Straus1952} observations, it was true that the girl of 5 threw poorly, but she could not do otherwise as her abilities to throw manifest in the body due to a by-product of her social and cultural status \cite{Bourdieu2000}. Girls are molded into the body of the socio-culturally prescribed female, just as boys are molded into the body of the socio-culturally prescribed male. 
%Only through equal representation of all groups in positive stratospheres of society can our intrinsic biases shift. Efforts to retroactively remove biases from language and vision models and datasets will continue to be necessary, but it will be a Sisyphean task until we address the root cause, societal perceptions of females in sports. Gender bias is only one facet of a larger biasing problem that exists \cite{Torralba2011}, \cite{Hendricks2018}. As a recurring issue in the field, it is clearly worthy of consideration. 


%In this study, gender bias is examined through a statistical analysis of Language and Vision datasets ManyNames \cite{Silberer2020} and VisualGenome \cite{Krishna2016}. In the first set of analyses, gender biases were conclusively determined to exist. VisualGenome is heavily biased with over twice as many male-named objects as female-named objects. ManyNames also displays this same image selection bias as it was derived from VisualGenome images, however, the bias is significantly smaller than what was seen in VisualGenome. The second analysis confirmed a human naming bias and our final study showed a replication of the human naming bias by the model, although results are inconclusive as to whether an amplification or a reduction of the bias existed. The findings show the need for more equal representation in Language and Vision data sets if biases and their consequences are to be mitigated. 

%As hypothesized, each study demonstrates a gender bias exists within the data sets. In our first analysis, the bias presents as an over-representation of images of males to females, while in the following two studies the gender bias is exemplified through the phenomenon of cross-classification. Humans use many names to identify objects, and the name chosen for the referent highlights the qualities being focused on. Naming images of females taxonomically instead of by a sports role name reflects how women in sports are viewed, perpetuating the narrative that males are athletes and females are not. 

%Humans are flawed creatures. We each possess our own biases and the insidious nature of implicit bias is why we can be so unaware of its very existence in our lives \cite{Haselton2015}. Sports are historically and culturally segregated \cite{Dennis2015} in addition to being one of the most observable manifestations of gender bias and discrimination. While in other fields, bias is visible in socioeconomic indicators such as salary and position, in sports the bias is at the bodily level \cite{Young1980}, \cite{Straus1952}, \cite{Bourdieu2000}. By using the sports discrepancies within the gender we are able to see the discrimination at the least abstract level. In Straus' \cite{Straus1952} observations, it was true that the girl of 5 threw poorly, but she could not do otherwise as her abilities to throw manifest in the body due to a by product of her social and cultural status \cite{Bourdieu2000}. Girls are molded into the body of the socio-culturally prescribed female, just as boys are molded into the body of the socio-culturally prescribed male. It is only through equal representation of all groups in positive stratospheres of society that our intrinsic biases can shift. Efforts to retroactively remove biases from language and vision models and datasets will continue to be a necessary, but it will be a Sisphean task until we address the root cause, societal perceptions of females in sports. Gender bias is only one facet of a larger biasing problem that exists \cite{Torralba2011}, \cite{Hendricks2018}. As a recurring issue in the field, it is clearly worthy of consideration.%


%In the subset of images of people playing sports, ManyNames has a bias from the human annotators who showed a tendency to name images of males playing sports with a sports role name far more frequently than images of females playing sports. In the final analysis of the model trained on ManyNames data, the results showed there was a replication of the bias towards naming more images of males with a sports name over images of females. The human bias against images of females playing sports, discussed in Analysis II, is also present once again in the human responses to the 89 selected images the model saw. Results were inconclusive as to whether an amplification or reduction in the bias was occurring when the model probabilities and the human percentages were compared across images of people playing sports by gender. It is suspected that reproducing this analysis with a larger sample set would in fact still yield the same bias towards images of males playing sports that was visible in the whole of ManyNames, and likely display amplification of said bias. Ultimately, based on the findings of this paper, it can be concluded that, as far as the datasets and model analyzed herein are concerned, when it comes to sports: A man with a tennis racket is a tennis player. A woman with a tennis racket is just a woman with a tennis racket.%

We call this set of factors ``sport-related gender bias'' . This sport-gender bias constitutes direct harm to women and especially young girls. Girls drop out of sports at twice the rate of boys. This trend continues until adulthood where the cycle continues as there are fewer female-athlete role models, directly contributing to representational harm, girls do not see their future selves as athletes to the same degree that boys do. 


==> for-final-version.tex <==
"The report also found that, at high schools across the county, only 60% of girls are participating in sports compared to 75% of their male peers." https://www.womenssportsfoundation.org/wp-content/uploads/2022/04/FINAL6_WSF-Title-IX-Infographic-2022.pdf

https://globalsportmatters.com/youth/2019/10/11/girls-play-sports-less-than-boys-miss-out-on-crucial-benefits/

During the 2015-16 school year, 52% of boys participated in high school sports, and 44% of girls did, even though schools offered similar opportunities, the  Women’s Sports Foundation (WSF) reported in its July 2019 report The State of High School Sports in America (https://www.womenssportsfoundation.org/research/article-and-report/recent-research/state-high-school-sports-report-evaluation-nations-popular-extracurricular-activity/)


Also found reports that say the same for the UK https://www.theguardian.com/education/2022/mar/07/uk-girls-lose-interest-in-sport-as-teenagers-women-in-sport-survey). So that shows that at least in the US, Canada (https://www.cbc.ca/sports/youth-sports-teenagers-female-male-participation-1.5607509), the UK, and Australia we see the same pattern of fewer girls participating.


==> intro-legacy.tex <==

%Current attempts to account for bias in NLP lack the normative reasoning required to properly address this dire issue \cite{Blodgett2020}.


%Biases are a problem in society and therefore a problem in AI through our human-created datasets. Computational models identify patterns and associations within the data they are trained on to best complete the assigned task. The models find biases within the datasets and produce biased results. These biased results have real-world impacts: people of color are disproportionately misidentified as criminals by facial recognition software, and women and minorities are not chosen for interviews by resume reviewing algorithms based on their gender or for having “non-white'' names. There is a moral and ethical responsibility to mitigate harmful outcomes of biased datasets and consequently biased models. 

%In this work, we analyze %sport-related gender bias two datasets developed for Language and Vision research: ManyNames \cite{Silberer2020}and VisualGenome \cite{Krishna2016}. We present three analyses. First, we check whether the two datasets contain balanced proportions of images of males and females, representing the two most common genders\footnote{While biological sex is assigned at birth based on the genitals as either male, female, or intersex, gender identity is more complex. We acknowledge the fluidity of gender and the existence of other genders beyond ‘female’ and ‘male’, however, for the purposes of this study – determining a naming bias and image selection bias - we chose to focus efforts on the two most prevalent gender identities on the spectrum at the time of writing this paper.}equally. In the second and the third analyses, we focus on ManyNames, investigating whether the naming annotations collected exhibit the sport-related gender bias we hypothesize, and whether this bias is reproduced – or even amplified – by a Language and Vision model trained to perform object classification. %

%Studies 2 and 3 investigate misrepresentation through human-naming behavior; i.e. how women are named differently than men when playing sports

%The phenomenon of cross-classification \cite{Silberer2020}, the human ability to refer to one object by more than a single name, demonstrates sport-related gender bias in our studies. For example, the subject in Figure \ref{fig:surfer_woman} can be called both "woman" and "surfer", however, in Study 2 'woman' is the name chosen most frequently by human annotators for this image. What makes her less of a surfer than the subject in Figure \ref{fig:surfer_man}? Cross-classification shows how the name chosen for an object is directly linked to aspects of the referent that the namer wants to highlight. In female athletes, the aspect most highlighted is their femininity. 

%In this paper, we examine whether a gender bias of similar nature is at play when speakers are tasked to produce names for images of men and women playing sports.

%We learn to name objects with different levels of specificity \cite{Rosch1975, Jolicoeur1984}. For example, we may refer to the same dog with the more general term "animal", or with a more specific term like "German Shepard". Often speakers produce different names for the same objects, encoding in their choice different aspects of the referent that they want to highlight. For example, the subject of Figure \ref{fig:surfer_woman} can be called both "woman" and "surfer". This phenomenon is called \textit{cross-classification} \cite{Silberer2020}.%



%Datasets with unbalanced classes can lead to inaccurate results, as models struggle to capture patterns and information for the minority classes in the data \cite{10.5555/555733}. This problem can cause real-world harm when the unequal distribution of training data systematically disfavors some social groups, unintentionally propagating biases, such as racial and gender stereotypes \cite{srinivasan-bisk-2022-worst}.
%\citet{Crawford2017} and \citet{Blodgett2020} define the term ``representational harm" for systems demeaning or even ignoring some social groups.%
%From Blodgett et al: 
% taxonomy of harms 
% allocational
%and representational harms (Barocas et al.,
%2017; Crawford, 2017). Allocational harms arise
%when an automated system allocates resources (e.g.,
%credit) or opportunities (e.g., jobs) unfairly to different
%social groups; representational harms arise
%when a system (e.g., a search engine) represents
%some social groups in a less favorable light than
%others, demeans them, or fails to recognize their
%existence altogether.
This problem touches Language \& Vision models as well, which are a specific type of AI models, dealing with tasks connecting words to visual inputs, such as images or videos. Typical Language \& Vision tasks are referring expression generation (REG) \cite{Kazemzadeh2014}, visual question-answering (VQA) \cite{Kafle2017}, and image captioning \cite{Wang2020}. 

%The phenomenon of cross-classification \cite{Silberer2020}, the human ability to refer to one object by more than a single name, demonstrates sport-related gender bias in our studies. For example, the subject in Figure \ref{fig:surfer_woman} can be called both "woman" and "surfer", however, in Study 2 'woman' is the name chosen most frequently by human annotators for this image. What makes her less of a surfer than the subject in Figure \ref{fig:surfer_man}? Cross-classification shows how the name chosen for an object is directly linked to aspects of the referent that the namer wants to highlight. In female athletes, the aspect most highlighted is their femininity.

Some biases are easier to spot and quantify (e.g.\ computing the number of Caucasian vs.\ non-Caucasian individuals in an image dataset), whereas some are more insidious (e.g.\ the association of women vs.\ men with specific jobs like nurse or computer scientist). 

In this paper, we examine two datasets developed for Language and Vision research: ManyNames \cite{Silberer2020}
and VisualGenome \cite{Krishna2016} for bias. In our first study, we focus on the invisibilization of women through an underrepresentation of female images within ManyNames and VisualGenome. We investigate whether the two datasets contain balanced proportions of images of males and females, representing the two most common genders\footnote{While biological sex is assigned at birth based on the genitals as either male, female, or intersex, gender identity is more complex. We acknowledge the fluidity of gender and the existence of other genders beyond ‘female’ and ‘male’, however, for the purposes of this study – determining a naming bias and image selection bias - we chose to focus efforts on the two most prevalent gender identities on the spectrum at the time of writing this paper.}. 

In our second analysis, we focus on ManyNames, investigating misrepresentation through human-naming behavior; i.e. how women are named differently than men when playing sports. In particular, we speculate that speakers more often choose a name to highlight the sport when their referent is a man. We call this ``\textbf{sport-related gender bias}''. Figure \ref{fig:surfers} shows qualitative evidence of this bias. \EG{explain the figure}. We hypothesize that this bias may exist because sport has long been stereotypically associated with masculinity and women have been thought physically incapable of performing well in this area \cite{Young1980}. \EG{Connect to referential choice?}

Finally, given that we find the hypothesized bias in the human naming annotations, in our third study, we analyze the predictions of a Language \& Vision model trained to perform object classification on ManyNames, checking whether it reproduces --or even amplifies-- the sport-related gender bias. 

In this work, we analyze sport-related gender bias two datasets developed for Language and Vision research: ManyNames \cite{Silberer2020}and VisualGenome \cite{Krishna2016}. We present three analyses. First, we check whether the two datasets contain balanced proportions of images of males and females, representing the two most common genders\footnote{While biological sex is assigned at birth based on the genitals as either male, female, or intersex, gender identity is more complex. We acknowledge the fluidity of gender and the existence of other genders beyond ‘female’ and ‘male’, however, for the purposes of this study – determining a naming bias and image selection bias - we chose to focus efforts on the two most prevalent gender identities on the spectrum at the time of writing this paper.}equally. In the second and the third analyses, we focus on ManyNames, investigating whether the naming annotations collected exhibit the sport-related gender bias we hypothesize, and whether this bias is reproduced – or even amplified – by a Language and Vision modeltrained to perform object classification. 



There is a relationship between language and social hierarchies \cite{Blodgett2020}. The names we use to refer to and categorize  objects directly mirror our conceptualization of them in society \cite{LaTourrette2020}, and are directly linked to the aspects of the referent that we want to highlight.
%humans are biased \cite{Haselton2015}, and therefore so are the annotations in our datasets \cite{Torralba2011, Wen2021}.
Since object naming is an integral component of the tasks that Language \& Vision models are trained to accomplish, they may learn and propagate stereotypical associations such as outputting the name `nurse' more often for images depicting women and the name `doctor' for images depicting men, which may be as harmful as non-representing minority classes. 


Figure \ref{fig:surfers} provides qualitative evidence exemplifying this naming bias in the object labels of images from the ManyNames dataset \cite{Silberer2020}: the person in panel \ref{fig:surfer_woman} --a woman surfing-- has been called `woman" more often than `surfer", while the person in panel \ref{fig:surfer_man} --a man surfing-- has been called `surfer" way more often than any other name.
Naming annotations collected in a free-naming task are listed, with response counts in parentheses. We can notice that the image in panel (a), depicting a woman surfing, received way less sports-related name (in this case, `surfer') than the image in panel (b), depicting a man surfing, supporting the hypothesis of a sports-related gender bias at play when speakers are tasked to name objects in pictures.%

